Rare-Seed Generation for Fuzzing

Starting with a random initial seed, fuzzers search for inputs that trigger bugs or vulnerabilities. However, fuzzers often fail to generate inputs for program paths guarded by restrictive branch conditions. In this paper, we show that by first identifying rare-paths in programs (i.e., program paths with path constraints that are unlikely to be satisfied by random input generation), and then, generating inputs/seeds that trigger rare-paths, one can improve the coverage of fuzzing tools. In particular, we present techniques 1) that identify rare paths using quantitative symbolic analysis, and 2) generate inputs that can explore these rare paths using path-guided concolic execution. We provide these inputs as initial seed sets to three state of the art fuzzers. Our experimental evaluation on a set of programs (that contain a lot of restrictive branch conditions) shows that the fuzzers achieve better coverage with the rare-path based seed set compared to a random initial seed.

==> methodology.tex <==
We generate rare seeds for the fuzzer using a combination of control flow extraction, dependency analysis, model counting and guided symbolic execution. First, we discuss how we find out the rare static paths those are difficult to cover for a fuzzer. TO find out the rare static paths we use branch selectivity based on control flow and data flow analysis and model counting. Then we use each rare static path to guide symbolic execution to generate a rare seed. My idea is that these rare seeds can help the fuzzer to easily explore the rare paths immediately and mutating the rare seeds can generate inputs that will explore comparatively less rare paths and hence the overall coverage of the fuzzer will be improved.

\subsection{Finding out Rare Static Paths}
We generate a list of rare static paths using probabilistic prioritization of paths. A path with lowest probability score is identified as the rarest path in the program for a fuzzer to explore. To compute path probability we use branch selectivity. Once, we have the selectivity score computed for all the branches in the program, we run a depth first search to compute probabilities for all the path in then program and choose $n$ number of rare static paths.

\subsubsection{Branch Selectivity}

\subsubsection{Probabilistic Path Prioritization}
Once we are done computing selectivity for all the program branches, we run a depth first search to traverse all the paths and compute probability of the paths. Here, instead of running  
\subsubsection{Rare Path Selection}

\subsection{Generating Rare Seeds}
\subsubsection{Static Path Guided Symbolic Execution}
\subsubsection{Rare Seed Construction}
